Towards an Accessible Mathematics Working Environment Based on Isabelle/VSCode

The paper collects preparatory work for interdisciplinary collaboration between three partners, between (1) expertise in improving accessibility of studies for impaired individuals, (2) expertise in developing educational mathematics software and (3) expertise in designing and implementing interactive proof assistants. The cooperation was started with the goal to develop an accessible mathematics working environment for education with reasonable efforts. The start was triggered by the lucky discovery that the upcoming Isabelle/VSCode is greatly accessible for blind users without further impairments; this is envisaged as the project's target group. Technical details are described to an extent necessary to understand essential details of efforts required for development. A survey of demand from practice of education with respect to (1) and (2) leads to a vision for educational math software, which necessarily is sketchy but suffices to guide development and which shall invite experts in didactics of mathematics to collaborate.

==> eptcsdata.tex <==
\providecommand{\firstpage}{92}
\providecommand{\publicationstatus}{J. Marcos, W. Neuper and P. Quaresma (Eds.): Theorem Proving Components\\ for Educational Software 2022 (ThEdu'22)\\
EPTCS 375, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.375.8}{10.4204/EPTCS.375.8}}
\pdfoutput=1

